HDR Video Reconstruction with Tri-Exposure Quad-Bayer Sensors

We propose a novel high dynamic range (HDR) video reconstruction method with new tri-exposure quad-bayer sensors. Thanks to the larger number of exposure sets and their spatially uniform deployment over a frame, they are more robust to noise and spatial artifacts than previous spatially varying exposure (SVE) HDR video methods. Nonetheless, the motion blur from longer exposures, the noise from short exposures, and inherent spatial artifacts of the SVE methods remain huge obstacles. Additionally, temporal coherence must be taken into account for the stability of video reconstruction. To tackle these challenges, we introduce a novel network architecture that divides-and-conquers these problems. In order to better adapt the network to the large dynamic range, we also propose LDR-reconstruction loss that takes equal contributions from both the highlighted and the shaded pixels of HDR frames. Through a series of comparisons and ablation studies, we show that the tri-exposure quad-bayer with our solution is more optimal to capture than previous reconstruction methods, particularly for the scenes with larger dynamic range and objects with motion.

==> acknowledgement.tex <==
\section*{Acknowledgements}
\label{sec:acknowledgements}
\noindent ADD ACK HERE

==> discussion.tex <==
%\section{Discussion}
%\label{sec:discussion}
%\mparagraph{Training Datasets}%
% in evaluation: R1, R3
%----------------------------------------------------
%R1 and R3 questioned the impact of the training dataset on accuracy presented in Table 1.
%Since our stereo-SR method requires a stereo image dataset, any ordinary SR dataset cannot be used like other methods. Instead, 
%We use a learning dataset that includes 60 images from the Middlebury dataset, while we use test images from other datasets (5 Middlebury images, 16 Tsukuba images, and 116 KITTI images) that are not used in the training process. To test the impact of the training dataset on accuracy, we attempted to train the original SRCNN method with the same training dataset that we used. The accuracy evaluation of the newly trained SRCNN network shows 31.39 for 5 Middlebury test images and 40.11 for 16 Tsukuba images. This accuracy is not significantly different from that of the original SRCNN model trained by the authors (the average PSNR of 31.48 for 5 Middlebury test images and 40.05 for 16 Tsukuba images, as shown in Table 1). This validates that the evaluation of our stereo-SR method with other methods is not affected by the training dataset.

%\mparagraph{Color space}%
%: R1, R3
%--------------------------
%R1 and R3 questioned the evaluation color space for accuracy. To be clear, we apply existing SR methods on each RGB channel, respectively, to obtain color SR images, rather than decomposing the input to luminance and chrominance. Even with our method, we use RGB input and output, since we trained our two-subnetwork architecture in an end-to-end manner. Note that we use luminance-chrominance decomposition only internally. Figure 4 is only for internal comparison to evaluate the impact of our second chrominance network. We will clarify this concern in the main text.


%\mparagraph{Downsampling scheme}
% for constructing dataset: R1
%------------------------------------------------
%We found that other SISR methods (SRCNN, VDSR, and PsyCo) use a built-in MATLAB implementation of bicubic downsampling for constructing the training and test datasets. We also use the same method for fairness in comparison.


%\mparagraph{Multiframe (video) SR}
% vs. our StereoSR: R1
%-----------------------------------
%Video SR and light-field super-resolution (LFSR) methods rely on short baseline characteristics for training networks. Those methods are inapplicable for our dual camera setup with a large disparity. For example, when we evaluated Liao's video super-resolution method with our stereo dataset, the results show the average PSNR of 24.77 for 5 Middlebury test images, which are even lower than that of bicubic upsampling. We found that those methods require a larger number of images with a small motion for proper operation.

%R. Liao, X. Tao, R. Li, Z. Ma, and J. Jia. Video super-resolution via deep draft-ensemble learning. In Proceedings of the IEEE International Conference on Computer Vision, pages 531–539, 2015


%\mparagraph{Directly combining stereo images}
% for SR: R3
%-------------------------------------------
%In Figure 5, we provide a plot, labeled "stereo learning." We trained a straightforward SR network that takes two stereo images as input and trained in an end-to-end regression manner. Even though it is better than a single-image stereo training, the accuracy of the direct "stereo learning" is significantly lower than the proposed method. It is the reason why the typical CNN network can find correspondences only with small disparity such as light-field images but often fails in finding correspondences in the dual camera stereo setup due to the wide disparity.


%\mparagraph{Jointly learning the two-subnetwork architecture}
%: R1, R3
%--------------------------------------------
%Our network consists of two different subnetworks: luminance SR and color reconstruction. We jointly trained the both networks in a single learning process in an end-to-end manner, to avoid any potential residual errors in two-network architecture.
%Our joint-learning approach is motivated to avoid any potential problem that the second chrominance networks learn from residuals of the first luminance channel. 
%Regarding training, the size of the original dataset is 26,000 patches. The augmentation multiplies the original size by six (by four 90-deg. rotations and horizontal/vertical flips), resulting in 156,000 patches. The total iteration is 50,000 with the batch size of 128, resulting in 6,400,000 training samples in total. We therefore trained our network with approximately 41 epochs.


==> evaluation.tex <==
\section{Evaluation}

==> final_result_figures.tex <==

\begin{table*}[htpb]
	\begin{center}
		\vspace{2mm}%
		\includegraphics[width=0.9\linewidth]{./figs/algorithm_comparison.pdf}%
	\end{center}
	\vspace{-6mm}
	\caption[]{\label{table:algorithm_comparison}%
Quantitative evaluation of our method with state-of-the-art SR algorithms for $\times$2, $\times$3 and $\times$4 magnification ratios on the Middlebury stereo dataset, Tsukuba dataset, and KITTI stereo dataset. Red color indicates the highest accuracy, and blue color presents the second highest accuracy regarding PSNR [dB] and SSIM.} 
	\vspace{0mm}
\end{table*}
\begin{figure*}[pht]
	\vspace{-3mm}
	\begin{center}
		\setlength\tabcolsep{1pt}
		\begin{tabular}{cccccc}
			\vspace{-2mm}
			\footnotesize\subfloat{Ground truth} &
			\footnotesize\subfloat{Bicubic} &
			\footnotesize\subfloat{SRCNN~\cite{dong2014learning}} &
			\footnotesize\subfloat{VDSR~\cite{kim2016accurate}} &
			\footnotesize\subfloat{PSyCo~\cite{Perezpellitero2016psyco}} &
			\footnotesize\subfloat{Our method} \\
			\vspace{-3mm}
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/GND_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/Bicubic_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/SRCNN_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/VDSR_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/PSyCo_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/SSRN_0.pdf}} \\
			\vspace{-3mm}
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/GND_cropped_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/Bicubic_cropped_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/SRCNN_cropped_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/VDSR_cropped_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/PSyCo_cropped_0.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/SSRN_cropped_0.pdf}} \\
			\vspace{-3mm}
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/GND_cropped_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/Bicubic_cropped_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/SRCNN_cropped_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/VDSR_cropped_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/PSyCo_cropped_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/motorcycle_color/SSRN_cropped_1.pdf}} \\
			\footnotesize\subfloat{(PSNR, SSIM)} &
			\footnotesize\subfloat{{(25.47 dB, 0.8528)}} &
			\footnotesize\subfloat{{(27.03 dB, 0.8995)}} &
			\footnotesize\subfloat{{(27.22 dB, 0.9045)}} &
			\footnotesize\subfloat{{\color{blue} (27.39 dB, 0.9050)}} &
			\footnotesize\subfloat{{\color{red} (28.58 dB, 0.9160)}} \\
			\vspace{-3mm}
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/GND_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/Bicubic_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/SRCNN_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/VDSR_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/PSyCo_1.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/SSRN_1.pdf}} \\
			\vspace{-3mm}
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/GND_cropped_2.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/Bicubic_cropped_2.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/SRCNN_cropped_2.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/VDSR_cropped_2.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/PSyCo_cropped_2.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/SSRN_cropped_2.pdf}} \\
			\vspace{-3mm}
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/GND_cropped_3.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/Bicubic_cropped_3.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/SRCNN_cropped_3.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/VDSR_cropped_3.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/PSyCo_cropped_3.pdf}} &
			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/kitti_2012_0013/SSRN_cropped_3.pdf}} \\
			\footnotesize\subfloat{(PSNR, SSIM)} &
			\footnotesize\subfloat{{(26.82 dB, 0.8920)}} &
			\footnotesize\subfloat{{(28.28 dB, 0.9240)}} &
			\footnotesize\subfloat{{\color{blue} (28.75 dB, 0.9237)}} &
			\footnotesize\subfloat{{(28.73 dB, 0.9264)}} &
			\footnotesize\subfloat{{\color{red} (29.20 dB, 0.9318)}} \\
%			\vspace{-3mm}
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/GND_2.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/Bicubic_2.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/SRCNN_2.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/VDSR_2.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/PSyCo_2.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/SSRN_2.pdf}} \\
%			\vspace{-3mm}
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/GND_cropped_4.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/Bicubic_cropped_4.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/SRCNN_cropped_4.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/VDSR_cropped_4.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/PSyCo_cropped_4.pdf}} &
%			\subfloat{\includegraphics[width = 0.15\linewidth]{./figs/results/state_of_art/pdf/cloth2_color/SSRN_cropped_4.pdf}} \\
%			\subfloat{(PSNR, SSIM)} &
%			\subfloat{{(32.00 dB, 0.8781)}} &
%			\subfloat{{(34.13 dB, 0.9287)}} &
%			\subfloat{{(34.26 dB, 0.9278)}} &
%			\subfloat{{\color{blue} (34.35 dB, 0.9301)}} &
%			\subfloat{{\color{red} (35.28 dB, 0.9406)}} \\
			
		\end{tabular}
	\end{center}
	\vspace{-5mm}
	\caption[]{\label{fig:results}%
		Results of super-resolution with the $\times$2 magnification factor. PSNR and SSIM values are shown under each result. The red color indicates the highest PSNR and SSIM values, and the blue color represents the second highest values.} 
	\vspace{-5mm}
\end{figure*}

